High Resolution UDF Meshing via Iterative Networks

Unsigned Distance Fields (UDFs) are a natural implicit representation for open surfaces but, unlike Signed Distance Fields (SDFs), are challenging to triangulate into explicit meshes. This is especially true at high resolutions where neural UDFs exhibit higher noise levels, which makes it hard to capture fine details. Most current techniques perform within single voxels without reference to their neighborhood, resulting in missing surface and holes where the UDF is ambiguous or noisy. We show that this can be remedied by performing several passes and by reasoning on previously extracted surface elements to incorporate neighborhood information. Our key contribution is an iterative neural network that does this and progressively improves surface recovery within each voxel by spatially propagating information from increasingly distant neighbors. Unlike single-pass methods, our approach integrates newly detected surfaces, distance values, and gradients across multiple iterations, effectively correcting errors and stabilizing extraction in challenging regions. Experiments on diverse 3D models demonstrate that our method produces significantly more accurate and complete meshes than existing approaches, particularly for complex geometries, enabling UDF surface extraction at higher resolutions where traditional methods fail.

==> figs/problem.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

% Temporary modification of the table column separation width
\setlength\mytabcolsep{\tabcolsep}
\setlength\tabcolsep{4pt}


\newcommand{\pblmimg}[1]{\includegraphics[width=0.3\linewidth]{#1}}


\begin{figure}
    \centering
    \begin{tabular}{ccc}
    	% Full or large portion of plane
%    	\pblmimg{figs/problem/} && \\
    	% Zoomed in over the inset
%    	\pblmimg{figs/problem/} && \\
    \end{tabular}
    \caption{\NT{TODO: UDF of the teaser plane, with zoom on top region. Zero-isosurface is discontinued, so baseline fails while we don't.}}
    \label{fig:problem}
    \vspace{-5mm}
\end{figure}


% Restore table column separation width
\setlength{\tabcolsep}{\mytabcolsep}


==> figs/teaser_gif.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

% Temporary modification of the table column separation width
\setlength\mytabcolsep{\tabcolsep}
\setlength\tabcolsep{4pt}


\newcommand{\teaserimg}[1]{\includegraphics[width=0.255\linewidth]{#1}}


\begin{figure}
    \centering
    \setlength\tabcolsep{8pt}
    \begin{tabular}{cc}
%    	\includegraphics[width=0.475\linewidth]{figs/problem/true_udf_old} & \includegraphics[width=0.475\linewidth]{figs/problem/neural_udf_old} \\
    	\includegraphics[width=0.3\linewidth]{figs/problem/true_udf_blue.jpg} & \includegraphics[width=0.3\linewidth]{figs/problem/neural_udf_blue.jpg} \\
    	True UDF & Neural UDF \\
    \end{tabular}
	\setlength\tabcolsep{2pt}
    \begin{tabular}{ccc|ccc}
    	% Baselines
    	% \teaserimg{figs/teaser/shapenet_planes_1_512_meshudf} & 
		\teaserimg{figs/teaser/shapenet_planes_1_512_nsdudf} & 
		% \teaserimg{figs/teaser/shapenet_planes_1_512_dmudf_tuned} &
    	% Ours over iterations
    	\teaserimg{figs/teaser/shapenet_planes_1_512_ours_r5} 
		% & \teaserimg{figs/teaser/shapenet_planes_1_512_ours_r1} & \teaserimg{figs/teaser/shapenet_planes_1_512_ours_r5} 
		\\
    	
    	% MeshUDF & NSD-UDF & DMUDF &
		Single-pass &
    	Ours (multi-pass) - iter. 6 \\
    \end{tabular}
    \vspace{-1mm}
    \caption{{\bf Avoiding holes in a plane cockpit.} (Top) Compared to the ground-truth UDF of a plane, an approximate neural UDF may fail to reach zero, shown in white, at the true surface location. This is clear in the UDF detail shown in the upper right corner, where the two white areas are disconnected. This yields disconnections and holes in the reconstructions, especially at high resolutions. (Bottom) This causes holes in the surfaces reconstructed by current methods. By leveraging neighboring \fs{surfaces}, our iterative method properly recovers the cockpit nevertheless.}
    \label{fig:teaser}
    \vspace{-6mm}
\end{figure}


% Restore table column separation width
\setlength{\tabcolsep}{\mytabcolsep}


%---------------
% OLD
%---------------
\iffalse

% Older version with reconstructions on two lines

    \begin{tabular}{ccc}
	    	% Baselines
	    	\teaserimg{figs/teaser/shapenet_planes_1_512_meshudf} & \teaserimg{figs/teaser/shapenet_planes_1_512_nsdudf} & \teaserimg{figs/teaser/shapenet_planes_1_512_dmudf_tuned} \\
	    	MeshUDF~\cite{Guillard22b} & NSD-UDF~\cite{Stella24} & DMUDF~\cite{Zhang23b} \\
	    	% Ours over iterations
	    	\teaserimg{figs/teaser/shapenet_planes_1_512_ours_r0} & \teaserimg{figs/teaser/shapenet_planes_1_512_ours_r1} & \teaserimg{figs/teaser/shapenet_planes_1_512_ours_r5} \\
	    	Ours - iter. 1 & Ours - iter. 2 & Ours - iter. 6 \\
	    \end{tabular}
\fi

==> tabs/filtering_strat_poster.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table}[!ht]
    \caption{ \textbf{Filtering and meshing times.} (a) Median L2 Chamfer Distance $\times 10^{-5}$ with 2M sample points (CD), Image Consistency (IC) and model inference times are reported at varying grid resolutions on an auto-decoder  trained on ShapeNet  cars. The times were  measured on an NVIDIA A100 GPU. Notice that our filtering strategies put the proposed pipeline in the same range as existing methods, without impacting its accuracy.
    }
    % \vspace{-5mm}
    % \begin{scriptsize}
        % \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \begin{subtable}{\columnwidth}
                \caption{Our filtering strategies speed up the method, maintaining the accuracy within run-to-run variance.}
                \label{tab:filtering_strat}
            \centering
            \resizebox{0.65\columnwidth}{!}{%
            \begin{tabular}{cc|cc|c} % <-- Removed two 'c' specifiers here
                Res. & Filtering & CD $\downarrow$ & IC $\uparrow$ & Inference time $\downarrow$ \\ 
                \midrule
                \multirow{3}{*}{256} 
                    & Without filtering & 5.26 & 89.2 & 7m\\
                    & Low confidence & 5.24 & 89.2 & 1.5m \\
                    & UDF $<0.1$ and low confidence & 5.24 & 89.2 & 30s\\
                    \toprule
                \multirow{3}{*}{512} 
                    & Without filtering & 8.91 & 88.9 & 1h\\
                    & Low confidence & 8.87 & 88.9 & 7m\\
                    & UDF $<0.1$ and low confidence & 8.88 & 88.9 & 2.5m\\
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
            \end{subtable}

            \vspace{2mm}
            \begin{subtable}{\columnwidth}
                \caption{Approximate UDF query and total meshing times at resolution 256. DCUDF makes multiple UDF queries at every iteration, making it difficult to measure the exact query time.}
                \label{tab:times}
                \centering
                \resizebox{0.65\columnwidth}{!}{%
                \setlength\tabcolsep{2pt} % default value: 6pt
                \begin{tabular}{c|ccccccc} % <-- Removed two 'c' specifiers here
                    Time & CAP &MeshUDF  & DCUDF  & NSD  & UNDC  & DMUDF  & Ours \\ 
                    \midrule
                        Query & 90s & 30s & / & 30s & 22s & 19s & 30s \\
                        Total & 3.5m & 35s & 25m & 35s & 30s & 20s & 1m \\
                    % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                    % \multicolumn{1}{c|}{Ours}        &  &  & & \\
                \end{tabular}
                }
                \end{subtable}
            % \vspace{-6mm}
        % \end{center}
    % \end{scriptsize}
\end{table}


==> tabs/main_results_all_poster.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
    \renewcommand{\arraystretch}{1.0}
    \caption{\small \textbf{Triangulating auto-decoder-based Neural Unsigned Distance Fields.} Median L2 Mesh Chamfer Distance $\times 10^{-5}$ with 2M sample points (CD), F1 score (F1) and Image Consistency (IC) are reported at varying grid resolutions. The best results are in bold. MGN* denotes halved resolution for our MGN experiments due to the lower complexity of the shapes. UNDC failed at resolution 512 due to its large GPU memory requirements.   }
%     \vspace{-5mm}

\begin{subtable}{\columnwidth}
    \caption{\textbf{Marching Cubes-based methods.}}
    \label{tab:main_results_mc}
    % \begin{scriptsize}
        \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{cc|ccc|ccc|ccc|ccc} % <-- Removed two 'c' specifiers here
                \multicolumn{2}{c}{} & \multicolumn{3}{c}{MGN$^2$ } & \multicolumn{3}{c}{ShapeNet cars }  & \multicolumn{3}{c}{ShapeNet chairs } & \multicolumn{3}{c}{ShapeNet planes } \\ 
                Res. & Method & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ \\ 
                \midrule
                \multirow{6}{*}{128} 
                    & CAP-UDF  & 16.2 & 69.4 & 79.4 & 53.9 & 53.3 & 83.2 & 378 & 50.9 & 70.3 & 14.0 & 69.5 & 80.6\\
                    & MeshUDF  & 2.45 & 82.9 & 94.1 & 11.3 & 57.7 & 88.6 & 7.43 & 67.6 & 88.0 & 6.82 & 74.6 & 81.0\\
                    & DCUDF  & 13500 & 2.50 & 2.76 & 6580 & 7.74 & 14.7 & 17000 & 15.9 & 13.9 & 1880 & 27.6 & 24.5\\
                    & DCUDF-T  & 90.8 & 2.86 & 87.3 & 50.3 & 58.0 & 87.3 & 214 & 64.1 & 82.9 & 144 & 68.8 & 77.2\\
                    & \nt{DCUDF-T-nocut}  & - & - & - & 11.4 & \textbf{61.7} & \textbf{89.4} & - & - & - & - & - & - \\
                    & NSD-UDF + MC  & \textbf{1.34} & \textbf{83.9} & \textbf{94.7} & 6.79 & 59.6 & 88.5 & 6.11 & \textbf{67.8} & 88.1 & 3.82 & \textbf{79.0} & \textbf{84.8}\\
                    & \textbf{Ours} + MC & 2.04 & 81.9 & 94.1 & \textbf{5.64} & 59.2 & 88.9 & \textbf{3.68} & 66.7 & \textbf{88.4} & \textbf{3.00} & 78.5 & \textbf{84.8}\\
                    \toprule
                \multirow{6}{*}{256} 
                    & CAP-UDF  & 1.66 & 86.8 & 91.8 & 34.0 & 61.2 & 87.6 & 114 & 70.5 & 82.0 & 5.50 & 83.7 & 85.4\\
                    & MeshUDF  & 0.958 & 89.7 & 95.0 & 13.6 & 62.3 & 88.6 & 27.8 & \textbf{72.9} & 87.3 & 3.47 & 85.8 & 85.2\\
                    & DCUDF  & 14400 & 4.76 & 3.71 & 346 & 52.6 & 78.2 & 3530 & 49.9 & 54.3 & 27.9 & 84.7 & 82.0\\
                    & DCUDF-T  & 4.63 & 86.8 & \textbf{95.4} & 347 & 52.6 & 78.2 & 3560 & 50.0 & 54.3 & 47.3 & 80.4 & 78.7\\
                    & \nt{DCUDF-T-nocut}  & - & - & - & 52.0 & 58.9 & 82.3 & - & - & - & - & - & - \\
                    & NSD-UDF + MC  & \textbf{0.808} & \textbf{90.0} & 95.2 & 10.2 & 62.0 & 87.9 & 10.9 & 72.3 & 86.2 & 2.91 & 87.3 & 86.0\\
                    & \textbf{Ours} + MC & 0.878 & 88.9 & 94.9 & \textbf{5.23} & \textbf{65.0} & \textbf{89.2} & \textbf{5.14} & \textbf{72.9} & \textbf{88.8} & \textbf{1.84} & \textbf{88.7} & \textbf{87.0}\\
                    
                    \toprule
                \multirow{6}{*}{512} 
                    & CAP-UDF  & 0.872 & 90.6 & 94.6 & 31.8 & 61.7 & 87.5 & 63.9 & 71.7 & 82.0 & 5.94 & 87.5 & 86.2\\
                    & MeshUDF  & 0.798 & 90.6 & \textbf{94.8} & 82.7 & 57.0 & 81.7 & 378 & 61.5 & 65.7 & 12.6 & 88.1 & 84.6\\
                    & DCUDF   & 4.37 & 88.3 & 91.1 & 223 & 56.5 & 84.2 & 2950 & 55.0 & 70.1 & 48.7 & 85.5 & 82.2\\
                    & DCUDF-T  & 4.38 & 88.2 & 91.1 & 223 & 56.5 & 84.2 & 2000 & 55.0 & 70.1 & 63.0 & 85.4 & 81.3\\
                    & \nt{DCUDF-T-nocut}  & - & - & - & 43.1 & 60.4 & 85.6 & - & - & - & - & - & - \\
                    & NSD-UDF + MC  & 0.784 & \textbf{90.8} & \textbf{94.8} & 56.9 & 58.8 & 83.8 & 295 & 64.7 & 75.7 & 10.0 & 89.4 & 85.1\\
                    & \textbf{Ours} + MC & \textbf{0.722} & 90.6 & \textbf{94.8} & \textbf{8.84} & \textbf{65.6} & \textbf{88.9} & \textbf{8.76} & \textbf{74.5} & \textbf{87.2} & \textbf{2.37} & \textbf{90.9} & \textbf{87.1}\\
                    
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
            %  \vspace{-2mm}
        \end{center}
    % \end{scriptsize}
\end{subtable}


\begin{subtable}{\columnwidth}
    \caption{\textbf{Dual Contouring-based methods.}}
    %  \vspace{-1mm}
    \label{tab:main_results_dc}
    % \begin{scriptsize}
        \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{cc|ccc|ccc|ccc|ccc} % <-- Removed two 'c' specifiers here
                \multicolumn{2}{c}{} & \multicolumn{3}{c}{MGN$^2$ } & \multicolumn{3}{c}{ShapeNet cars }  & \multicolumn{3}{c}{ShapeNet chairs } & \multicolumn{3}{c}{ShapeNet planes } \\ 
                Res. & Method & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ \\ 
                \midrule
                
                \multirow{5}{*}{128} 
                    & UNDC  & 1.09 & 87.1 & 94.1 & 13.5 & 61.7 & 86.4 & 29.9 & 69.4 & 81.9 & 2.50 & 82.0 & 86.1\\ 
                    & DualMesh-UDF   & 216 & 68.1 & 68.4 & 952 & 34.4 & 45.5 & 7930 & 12.1 & 9.08 & 112 & 74.3 & 76.1\\ 
                    & DualMesh-UDF-T  & 0.806 & 89.9 & 95.4 & 5.56 & 63.5 & 89.5 & 5.34 & \textbf{75.1} & 89.1 & 1.96 & 84.3 & 87.5\\
                    & NSD-UDF + DualMesh-UDF  & \textbf{0.760} & 90.4 & \textbf{95.0} & 6.34 & 65.7 & 89.1 & 5.50 & 72.8 & 89.2 & 2.08 & 87.1 & 86.6\\ 
                    & \textbf{Ours} + DualMesh-UDF & 0.787 & \textbf{90.5} & 94.9 & \textbf{4.80} & \textbf{66.2} & \textbf{89.7} & \textbf{3.39} & 72.8 & \textbf{89.8} & \textbf{1.56} & \textbf{87.7} & \textbf{88.2}\\
                    \toprule
                
                \multirow{5}{*}{256} 
                    & UNDC   & 0.931 & 89.1 & 91.5 & 82.4 & 52.3 & 71.4 & 293 & 54.2 & 57.8 & 11.6 & 83.6 & 80.7\\ 
                    & DualMesh-UDF  & 176 & 66.3 & 66.4 & 846 & 34.0 & 45.1 & 8280 & 12.4 & 9.26 & 105 & 77.9 & 76.0\\ 
                    & DualMesh-UDF-T  & 0.722 & \textbf{91.2} & \textbf{95.1} & 10.6 & 64.3 & 87.0 & 22.8 & \textbf{72.2} & 84.1 & 2.43 & 88.2 & 87.0\\
                    & NSD-UDF + DualMesh-UDF  & 0.671 & 91.0 & 94.6 & 10.5 & 64.9 & 87.2 & 14.6 & 70.7 & 84.4 & 2.78 & 88.9 & 85.6\\ 
                    & \textbf{Ours} + DualMesh-UDF & \textbf{0.662} & \textbf{91.2} & 94.7 & \textbf{5.48} & \textbf{65.7} & \textbf{88.8} & \textbf{4.97} & 71.9 & \textbf{86.4} & \textbf{1.87} & \textbf{90.0} & \textbf{87.5}\\
                    \toprule
                
                \multirow{5}{*}{512} 
                    & UNDC  & 2.39 & 84.8 & 82.8 & - & - & - & - & - & - & - & - & -\\ 
                    & DualMesh-UDF   & 167 & 63.7 & 63.9 & 870 & 32.5 & 43.0 & 8190 & 11.8 & 9.07 & 111 & 77.6 & 74.2\\ 
                    & DualMesh-UDF-T  & 0.827 & \textbf{90.2} & \textbf{93.2} & 37.8 & 58.2 & 79.3 & 72.7 & 63.7 & 72.5 & 4.77 & 89.0 & 84.0\\
                    & NSD-UDF + DualMesh-UDF  & 0.787 & 89.7 & 92.5 & 60.5 & 57.5 & 79.9 & 296 & 62.5 & 68.0 & 9.95 & 87.6 & 83.3\\ 
                    & \textbf{Ours} + DualMesh-UDF & \textbf{0.726} & 89.7 & 92.8 & \textbf{9.65} & \textbf{63.0} & \textbf{85.6} & \textbf{10.1} & \textbf{70.4} & \textbf{81.9} & \textbf{2.51} & \textbf{90.1} & \textbf{85.8}\\
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
            \vspace{-2mm}
        \end{center}
    % \end{scriptsize}
\end{subtable}

\end{table*}


==> tabs/main_results_dc.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
    \renewcommand{\arraystretch}{1.0}
    \caption{\small \textbf{Triangulating Neural Unsigned Fields using Dual Contouring-based methods.} Median L2 Chamfer Distance $\times 10^{-5}$ with 2M sample points (CD), F1 score (F1) and Image Consistency (IC) are reported at varying grid resolutions. The best results are in bold. UNDC failed at resolution 512 due to its large GPU memory requirements. MGN* denotes halved resolution for our MGN experiments due to the lower complexity of the shapes.
    }
     \vspace{-1mm}
    \label{tab:main_results_dc}
    % \begin{scriptsize}
        \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{cc|ccc|ccc|ccc|ccc} % <-- Removed two 'c' specifiers here
                \multicolumn{2}{c}{} & \multicolumn{3}{c}{MGN*~\cite{Bhatnagar19}} & \multicolumn{3}{c}{ShapeNet cars~\cite{Chang15}}  & \multicolumn{3}{c}{ShapeNet chairs~\cite{Chang15}} & \multicolumn{3}{c}{ShapeNet planes~\cite{Chang15}} \\ 
                Res. & Method & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ \\ 
                \midrule
                
                \multirow{5}{*}{128} 
                    & UNDC~\cite{Chen22b} & 1.09 & 87.1 & 94.1 & 13.5 & 61.7 & 86.4 & 29.9 & 69.4 & 81.9 & 2.50 & 82.0 & 86.1\\ 
                    & DualMesh-UDF~\cite{Zhang23b}  & 216 & 68.1 & 68.4 & 952 & 34.4 & 45.5 & 7930 & 12.1 & 9.08 & 112 & 74.3 & 76.1\\ 
                    & DualMesh-UDF-T~\cite{Zhang23b} & 0.806 & 89.9 & 95.4 & 5.56 & 63.5 & 89.5 & 5.34 & \textbf{75.1} & 89.1 & 1.96 & 84.3 & 87.5\\
                    & NSD-UDF + DualMesh-UDF~\cite{Stella24} & \textbf{0.760} & 90.4 & \textbf{95.0} & 6.34 & 65.7 & 89.1 & 5.50 & 72.8 & 89.2 & 2.08 & 87.1 & 86.6\\ 
                    & \textbf{Ours} + DualMesh-UDF & 0.787 & \textbf{90.5} & 94.9 & \textbf{4.80} & \textbf{66.2} & \textbf{89.7} & \textbf{3.39} & 72.8 & \textbf{89.8} & \textbf{1.56} & \textbf{87.7} & \textbf{88.2}\\
                    \toprule
                
                \multirow{5}{*}{256} 
                    & UNDC~\cite{Chen22b}  & 0.931 & 89.1 & 91.5 & 82.4 & 52.3 & 71.4 & 293 & 54.2 & 57.8 & 11.6 & 83.6 & 80.7\\ 
                    & DualMesh-UDF~\cite{Zhang23b} & 176 & 66.3 & 66.4 & 846 & 34.0 & 45.1 & 8280 & 12.4 & 9.26 & 105 & 77.9 & 76.0\\ 
                    & DualMesh-UDF-T~\cite{Zhang23b} & 0.722 & \textbf{91.2} & \textbf{95.1} & 10.6 & 64.3 & 87.0 & 22.8 & \textbf{72.2} & 84.1 & 2.43 & 88.2 & 87.0\\
                    & NSD-UDF + DualMesh-UDF~\cite{Stella24} & 0.671 & 91.0 & 94.6 & 10.5 & 64.9 & 87.2 & 14.6 & 70.7 & 84.4 & 2.78 & 88.9 & 85.6\\ 
                    & \textbf{Ours} + DualMesh-UDF & \textbf{0.662} & \textbf{91.2} & 94.7 & \textbf{5.48} & \textbf{65.7} & \textbf{88.8} & \textbf{4.97} & 71.9 & \textbf{86.4} & \textbf{1.87} & \textbf{90.0} & \textbf{87.5}\\
                    \toprule
                
                \multirow{5}{*}{512} 
                    & UNDC~\cite{Chen22b} & 2.39 & 84.8 & 82.8 & - & - & - & - & - & - & - & - & -\\ 
                    & DualMesh-UDF~\cite{Zhang23b}  & 167 & 63.7 & 63.9 & 870 & 32.5 & 43.0 & 8190 & 11.8 & 9.07 & 111 & 77.6 & 74.2\\ 
                    & DualMesh-UDF-T~\cite{Zhang23b} & 0.827 & \textbf{90.2} & \textbf{93.2} & 37.8 & 58.2 & 79.3 & 72.7 & 63.7 & 72.5 & 4.77 & 89.0 & 84.0\\
                    & NSD-UDF + DualMesh-UDF~\cite{Stella24} & 0.787 & 89.7 & 92.5 & 60.5 & 57.5 & 79.9 & 296 & 62.5 & 68.0 & 9.95 & 87.6 & 83.3\\ 
                    & \textbf{Ours} + DualMesh-UDF & \textbf{0.726} & 89.7 & 92.8 & \textbf{9.65} & \textbf{63.0} & \textbf{85.6} & \textbf{10.1} & \textbf{70.4} & \textbf{81.9} & \textbf{2.51} & \textbf{90.1} & \textbf{85.8}\\
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
            \vspace{-2mm}
        \end{center}
    % \end{scriptsize}
\end{table*}


==> tabs/main_results_mc.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
    \renewcommand{\arraystretch}{1.0}
    \caption{\small \textbf{Triangulating Neural Unsigned Fields using Marching Cubes-based methods.} Median L2 Chamfer Distance $\times 10^{-5}$ with 2M sample points (CD), F1 score (F1) and Image Consistency (IC) are reported at varying grid resolutions. The best results are in bold. MGN* denotes halved resolution for our MGN experiments due to the lower complexity of the shapes.    }
%     \vspace{-5mm}
    \label{tab:main_results_mc}
    % \begin{scriptsize}
        \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{cc|ccc|ccc|ccc|ccc} % <-- Removed two 'c' specifiers here
                \multicolumn{2}{c}{} & \multicolumn{3}{c}{MGN*~\cite{Bhatnagar19}} & \multicolumn{3}{c}{ShapeNet cars~\cite{Chang15}}  & \multicolumn{3}{c}{ShapeNet chairs~\cite{Chang15}} & \multicolumn{3}{c}{ShapeNet planes~\cite{Chang15}} \\ 
                Res. & Method & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ & CD $\downarrow$ & F1 $\uparrow$ & IC $\uparrow$ \\ 
                \midrule
                \multirow{6}{*}{128} 
                    & CAP-UDF~\cite{Zhou24} & 16.2 & 69.4 & 79.4 & 53.9 & 53.3 & 83.2 & 378 & 50.9 & 70.3 & 14.0 & 69.5 & 80.6\\
                    & MeshUDF~\cite{Guillard22b} & 2.45 & 82.9 & 94.1 & 11.3 & 57.7 & 88.6 & 7.43 & 67.6 & 88.0 & 6.82 & 74.6 & 81.0\\
                    & DCUDF~\cite{Hou23a} & 13500 & 2.50 & 2.76 & 6580 & 7.74 & 14.7 & 17000 & 15.9 & 13.9 & 1880 & 27.6 & 24.5\\
                    & DCUDF-T~\cite{Hou23a} & 90.8 & 2.86 & 87.3 & 50.3 & 58.0 & 87.3 & 214 & 64.1 & 82.9 & 144 & 68.8 & 77.2\\
                    & NSD-UDF + MC~\cite{Stella24} & \textbf{1.34} & \textbf{83.9} & \textbf{94.7} & 6.79 & \textbf{59.6} & 88.5 & 6.11 & \textbf{67.8} & 88.1 & 3.82 & \textbf{79.0} & \textbf{84.8}\\
                    & \textbf{Ours} + MC & 2.04 & 81.9 & 94.1 & \textbf{5.64} & 59.2 & \textbf{88.9} & \textbf{3.68} & 66.7 & \textbf{88.4} & \textbf{3.00} & 78.5 & \textbf{84.8}\\
                    \toprule
                \multirow{6}{*}{256} 
                    & CAP-UDF~\cite{Zhou24} & 1.66 & 86.8 & 91.8 & 34.0 & 61.2 & 87.6 & 114 & 70.5 & 82.0 & 5.50 & 83.7 & 85.4\\
                    & MeshUDF~\cite{Guillard22b} & 0.958 & 89.7 & 95.0 & 13.6 & 62.3 & 88.6 & 27.8 & \textbf{72.9} & 87.3 & 3.47 & 85.8 & 85.2\\
                    & DCUDF~\cite{Hou23a} & 14400 & 4.76 & 3.71 & 346 & 52.6 & 78.2 & 3530 & 49.9 & 54.3 & 27.9 & 84.7 & 82.0\\
                    & DCUDF-T~\cite{Hou23a} & 4.63 & 86.8 & \textbf{95.4} & 347 & 52.6 & 78.2 & 3560 & 50.0 & 54.3 & 47.3 & 80.4 & 78.7\\
                    & NSD-UDF + MC~\cite{Stella24} & \textbf{0.808} & \textbf{90.0} & 95.2 & 10.2 & 62.0 & 87.9 & 10.9 & 72.3 & 86.2 & 2.91 & 87.3 & 86.0\\
                    & \textbf{Ours} + MC & 0.878 & 88.9 & 94.9 & \textbf{5.23} & \textbf{65.0} & \textbf{89.2} & \textbf{5.14} & \textbf{72.9} & \textbf{88.8} & \textbf{1.84} & \textbf{88.7} & \textbf{87.0}\\
                    
                    \toprule
                \multirow{6}{*}{512} 
                    & CAP-UDF~\cite{Zhou24} & 0.872 & 90.6 & 94.6 & 31.8 & 61.7 & 87.5 & 63.9 & 71.7 & 82.0 & 5.94 & 87.5 & 86.2\\
                    & MeshUDF~\cite{Guillard22b} & 0.798 & 90.6 & \textbf{94.8} & 82.7 & 57.0 & 81.7 & 378 & 61.5 & 65.7 & 12.6 & 88.1 & 84.6\\
                    & DCUDF~\cite{Hou23a}  & 4.37 & 88.3 & 91.1 & 223 & 56.5 & 84.2 & 2950 & 55.0 & 70.1 & 48.7 & 85.5 & 82.2\\
                    & DCUDF-T~\cite{Hou23a} & 4.38 & 88.2 & 91.1 & 223 & 56.5 & 84.2 & 2000 & 55.0 & 70.1 & 63.0 & 85.4 & 81.3\\
                    & NSD-UDF + MC~\cite{Stella24} & 0.784 & \textbf{90.8} & \textbf{94.8} & 56.9 & 58.8 & 83.8 & 295 & 64.7 & 75.7 & 10.0 & 89.4 & 85.1\\
                    & \textbf{Ours} + MC & \textbf{0.722} & 90.6 & \textbf{94.8} & \textbf{8.84} & \textbf{65.6} & \textbf{88.9} & \textbf{8.76} & \textbf{74.5} & \textbf{87.2} & \textbf{2.37} & \textbf{90.9} & \textbf{87.1}\\
                    
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
             \vspace{-2mm}
        \end{center}
    % \end{scriptsize}
\end{table*}


==> tabs/supp_activation.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table}[!htb]
    \renewcommand{\arraystretch}{1.0}
    \caption{\small \textbf{.} Median Image Consistency (IC $\uparrow$) for Cars at 512. *Resolution is halved.
    }
    % \vspace{-5mm}
    \label{tab:training_iterations}
    % \begin{scriptsize}
        % \begin{center}
            % \setlength{\tabcolsep}{3pt}
            \resizebox{\columnwidth}{!}{%
            \begin{tabular}{c|ccc} % <-- Removed two 'c' specifiers here
                Function & \multicolumn{3}{c}{1 iter.} & \multicolumn{3}{c}{2 iter.} & \multicolumn{3}{c}{5 iter.} \\
                & & First pass & Last pass & Last+1 pass & First pass & Last pass & Last+1 pass & First pass & Last pass & Last+1 pass\\
                \midrule
                % \multirow{6}{*}{512} 
                    Identity & 87.0 & 88.6 & 86.7 & 87.6 & 88.2 & 88.1 & - & - & - \\
                    Softmax & 86.5 & 87.1 & 87.3 & 87.5 & 87.8 & 87.8 & - & - & - \\
                    Sigmoid & 87.6 & 88.5 & 88.9 & - & - & - & 87.2 & 88.0 & - \\
                    Sigmoid + Random $r$ & 87.9 & 88.5 & 88.8 & - & - & - & 87.8 & 88.9 & - \\
                    \toprule
                % \multicolumn{1}{c|}{MeshUDF\cite{Guillard22b}}        &  &  &  &  \\
                % \multicolumn{1}{c|}{Ours}        &  &  & & \\
            \end{tabular}
            }
            % \vspace{-6mm}
        % \end{center}
    % \end{scriptsize}
\end{table}

